Tri-Stack-PIM: A Heterogeneous Multi-Die 3D-Integrated Processing-in-Memory Architecture for Efficient LLM Inference

Large language model (LLM) inference during autoregressive decoding is fundamentally memory-bandwidth-bound. Existing three-dimensional (3D) stacked processing-in-memory (PIM) architectures alleviate the off-chip bandwidth wall, yet remain constrained by several limitations: physical layer (PHY), controllers, and direct memory access (DMA) engines compete with arithmetic units for advanced-node base-die area; hybrid-bonding keep-out zones fragment the base-die floorplan and impede physical design; compute tiles built in a dynamic random access memory (DRAM) process are restricted to low logic density, capping achievable throughput; and nonlinear operations offloaded to the host reintroduce a communication bottleneck. We present Tri-Stack-PIM, a heterogeneous three-die architecture that resolves these tensions by dedicating a top DRAM die to storage, a middle buffer die on a mature process node to PHYs, DMA engines, and near-memory compute units, and a bottom base die on an advanced node exclusively to single-instruction-multiple-data (SIMD) multiply-accumulate (MAC) arrays. We further introduce a Unified Buffer-Aware Ready-based (UBAR) hardware out-of-order micro-operation scheduler that enforces cross-die dependency correctness at runtime while maximizing issue-slot utilization through a multi-term priority function, recovering up to 90% of the cycles that an in-order policy would forfeit. A joint architecture-dataflow co-exploration identifies Pareto-optimal configurations that reduce the energy-delay product (EDP) by 33-66x over naive parameter selection. Evaluated across multi-head, grouped-query, and multi-query attention (MHA, GQA, MQA) mechanisms with batch sizes 1-32, Tri-Stack-PIM achieves geometric-mean speedups of 4.95x, 2.57x, and 1.68x across all three attention mechanisms and batch sizes over a graphics processing unit (GPU) baseline, AttAcc, and H2-LLM, respectively.

==> doc/acknowledge.tex <==
\section*{Acknowledgment}
This work was supported in part by the National Natural Science Foundation of China (Grant No. 62404021), the Beijing Natural Science Foundation (Grant No. L2603021), the Fundamental Research Funds for the BUPT (Grant No. 2025AI4S20), and the Research Initiation Project for Introduced Talents of BUPT (Grant No. 510124058).

==> doc/backgrounds.tex <==
% fig1
\begin{figure*}[!t]
    \centering
    \includegraphics[width=\textwidth]{fig1.pdf}
    \caption{Overview of the proposed three-tier TriPIM architecture, motivated by multi-factor co-design trade-offs across process scaling, HB I/O provisioning, and controller/PHY integration.
    The top DRAM die provides bank-level storage, the middle buffer die integrates the controller and vector-processing units for near-memory operations, and the bottom base die contains GEMM-oriented compute engines and local buffers.
    The left and right panels further illustrate the detailed microarchitecture of the buffer-die vector engine and the base-die compute core, respectively.}
    \Description{TriPIM overview with three stacked dies: DRAM storage on top, a middle buffer die with control and vector engines, and a base die with GEMM compute cores and local buffers.}
    \label{fig1}
\end{figure*}

\section{Background}
\label{sec:background}



\subsection{Transformer-based Large Language Model}

Autoregressive decoding generates tokens one at a time: each step
must reload the full model weights and the ever-growing KV cache from DRAM
while performing comparatively few arithmetic operations per fetched byte.
This fundamental imbalance yields a vanishingly low arithmetic intensity,
rendering the decoding phase inherently memory-bound. Compounding this bottleneck, the Softmax operator mandates a strict global
reduction over the entire attention sequence. Numerically stable evaluation
via the online Softmax algorithm requires iteratively propagating a running
maximum $m$ and a normalization accumulator $l$ across successive key-value
tile iterations $j$:
$$m^{(j)} = \max\!\left(m^{(j-1)},\, \max\bigl(S^{(j)}\bigr)\right)$$
$$l^{(j)} = l^{(j-1)} \cdot e^{\,m^{(j-1)} - m^{(j)}} + \cdots$$

A range of alternative choices has been proposed to attack this challenge—more advanced NPU microarchitectures~\cite{jouppi2017tpu, wang2021spatten}, and faster host-device fabrics such as PCIe~6.0~\cite{pcisig2022pcie6}, NVLink~\cite{foley2017nvlink}, and CXL~\cite{sharma2023cxl}. These efforts, however, treat the symptoms: they widen the data path but leave the memory-bound nature of decoding fundamentally intact.


\subsection{3D-Stacked Processing-in-Memory Architecture}
Processing-in-memory (PIM) has emerged as a promising paradigm for LLM
acceleration~\cite{seo2024ianus,heo2024neupims,park2024attacc,li2025h2,wu2024pim}, placing computation directly within the memory die. By bringing
low-arithmetic-intensity operations closer to where data resides, PIM
eliminates costly off-chip data movement and fully exploits the abundant
internal memory bandwidth that is otherwise inaccessible across the
chip boundary.

The rapid maturation of 3D integration has further accelerated the evolution
of PIM architectures~\cite{he2026tau,tsai2020soic_hbm}. In particular,
hybrid bonding (HB) realizes ultra-dense, low-parasitic vertical
interconnects between stacked dies~\cite{fujun2020stacked,wang2023135}.
Beyond logic-to-memory integration, recent prototypes demonstrate that HB
can bond multiple DRAM layers through mini-TSVs, forming deeply stacked
near-memory structures with high vertical bandwidth~\cite{wang2023135,wang2025_3duam}. Compared with conventional microbump packaging or off-chip interfaces, hybrid bonding delivers unprecedented vertical bandwidth, allowing the logic die to access the stacked DRAM dies at extremely high
throughput~\cite{li2025h2,li2026hardware}.

==> doc/related.tex <==
% \section{Related Work}
% \label{sec:related}

% \noindent\textbf{DRAM-Process PIM.}
% AttAcc~\cite{park2024attacc} places attention logic in GDDR6 banks to exploit internal bandwidth.
% Kwon et al.~\cite{kwon20221ynm} demonstrate a 1ynm GDDR6 accelerator-in-memory with TFLOPS-scale MAC.
% Both are constrained by DRAM-process logic density: complex reduction operators such as softmax require either external execution or area-inefficient DRAM-process circuits.

% \noindent\textbf{Hybrid Host-PIM Partitioning.}
% NeuPIMs~\cite{heo2024neupims} keeps the host NPU responsible for reduction and normalization while DRAM-side PIM handles matrix operations.
% This avoids density constraints but reintroduces round-trip data movement for every reduction step, partially negating near-memory bandwidth benefits and constraining pipeline overlap.

% \noindent\textbf{Hybrid-Bonding-Based PIM.}
% H$^2$-LLM~\cite{li2025h2} and Li et al.~\cite{li2026hardware} place advanced-node logic beneath DRAM via HB, demonstrating meaningful throughput gains.
% However, both couple host-facing PHY, HB controllers, DMA, and dense compute on a single logic die.
% As HB interface widths grow to deliver more bandwidth, this coupling creates interface-versus-compute pressure on the advanced-node die budget.
% Tri-Stack-PIM breaks this coupling with a dedicated mature-node Buffer Die.

% \noindent\textbf{Dynamic Scheduling in Memory Systems.}
% Out-of-order DRAM scheduling exploits bank-level parallelism by reordering requests to minimize row-activation penalties~\cite{luo2023ramulator}.
% The UBAR scheduler in Tri-Stack-PIM extends this principle to the cross-die execution pipeline, simultaneously reordering micro-operations spanning DRAM banks, HB links, SRE datapaths, and Base-Die compute tiles.
% This hardware-resident cross-die scheduler is uniquely enabled by the Buffer Die's cycle-level visibility into all resources in the 3D stack.

